First 100 days of pandemic; an interplay of pharmaceutical, behavioral and digital interventions -- A study using agent based modeling

Pandemics, notably the recent COVID-19 outbreak, have impacted both public health and the global economy. A profound understanding of disease progression and efficient response strategies is thus needed to prepare for potential future outbreaks. In this paper, we emphasize the potential of Agent-Based Models (ABM) in capturing complex infection dynamics and understanding the impact of interventions. We simulate realistic pharmaceutical, behavioral, and digital interventions that mirror challenges in real-world policy adoption and suggest a holistic combination of these interventions for pandemic response. Using these simulations, we study the trends of emergent behavior on a large-scale population based on real-world socio-demographic and geo-census data from Kings County in Washington. Our analysis reveals the pivotal role of the initial 100 days in dictating a pandemic's course, emphasizing the importance of quick decision-making and efficient policy development. Further, we highlight that investing in behavioral and digital interventions can reduce the burden on pharmaceutical interventions by reducing the total number of infections and hospitalizations, and by delaying the pandemic's peak. We also infer that allocating the same amount of dollars towards extensive testing with contact tracing and self-quarantine offers greater cost efficiency compared to spending the entire budget on vaccinations.

==> 8_config.tex <==
\subsection{Customizable configuration file}
Following is the config file that we used:
{\fontfamily{qcr}\selectfont
\newline
ADULT\_Upper\_Index: 6 \newline
CHILD\_Upper\_Index: 1 \newline
R: 5.02 \newline
age\_groups\_to\_ix\_dict: \newline
  AGE\_0\_9: 0 \newline
  AGE\_10\_19: 1 \newline
  AGE\_20\_29: 2 \newline
  AGE\_30\_39: 3 \newline
  AGE\_40\_49: 4 \newline
  AGE\_50\_59: 5 \newline
  AGE\_60\_69: 6 \newline
  AGE\_70\_79: 7 \newline
  AGE\_80: 8 \newline
age\_ix\_pop\_dict: \newline
  0: 278073 \newline
  1: 258328 \newline
  2: 317005 \newline
  3: 359688 \newline
  4: 323457 \newline
  5: 307938 \newline
  6: 229274 \newline
  7: 109487 \newline
  8: 69534 \newline
age\_ix\_prob\_list: \newline
- 0.12343526942662945 \newline
- 0.11467055873976377 \newline
- 0.1407169972798102 \newline
- 0.15966377602113652 \newline
- 0.14358100909807597 \newline
- 0.13669219951846248 \newline
- 0.1017736276536055 \newline
- 0.048600753556488324 \newline
- 0.03086580870602774 \newline
app\_user\_agewise\_probs\_dict: \newline
  AGE\_0\_9: 0.09 \newline
  AGE\_10\_19: 0.8 \newline
  AGE\_20\_29: 0.97 \newline
  AGE\_30\_39: 0.96 \newline
  AGE\_40\_49: 0.94 \newline
  AGE\_50\_59: 0.86 \newline
  AGE\_60\_69: 0.7 \newline
  AGE\_70\_79: 0.48 \newline
  AGE\_80: 0.32 \newline
debug: false \newline
genrerated\_params\_file\_name: generated\_params.yaml \newline
households\_sizes\_list: \newline
- 1 \newline
- 2 \newline
- 3 \newline
- 4 \newline
- 5 \newline
- 6 \newline
households\_sizes\_prob\_list: \newline
- 0.3404992742325125 \newline
- 0.3175985424643815 \newline
- 0.143990614165864 \newline
- 0.11976146407425071 \newline
- 0.04672432112547242 \newline
- 0.03142578393751882 \newline
num\_agents: 100000 \newline
num\_runs: 10 \newline
num\_stages: 11 \newline
num\_steps: 180 \newline
occupation\_ix\_to\_occupations\_dict: \newline
  AGRICULTURE: 0 \newline
  ART: 16 \newline
  CHILD: 20 \newline
  CONSTRUCTION: 3 \newline
  EDUCATION: 14 \newline
  ELDERLY: 19 \newline
  ENTERPRISEMANAGEMENT: 12 \newline
  FINANCEINSURANCE: 9 \newline
  FOOD: 17 \newline
  HEALTHCARE: 15 \newline
  INFORMATION: 8 \newline
  MANUFACTURING: 4 \newline
  MINING: 1 \newline
  OTHER: 18 \newline
  REALESTATERENTAL: 10 \newline
  RETAILTRADE: 6 \newline
  SCIENTIFICTECHNICAL: 11 \newline
  TRANSPORTATION: 7 \newline
  UTILITIES: 2 \newline
  WASTEMANAGEMENT: 13 \newline
  WHOLESALETRADE: 5 \newline
occupations\_sizes\_prob\_list: \newline
- 0.002074760790673804 \newline
- 0.0003245727393860931 \newline
- 0.001516673098112025 \newline
- 0.05915129446861781 \newline
- 0.08219465441221938 \newline
- 0.04930452985090788 \newline
- 0.13041196995040874 \newline
- 0.04084346122908182 \newline
- 0.09747122874002898 \newline
- 0.03305945551618415 \newline
- 0.02318190345213374 \newline
- 0.10423168231738673 \newline
- 0.024660222697601267 \newline
- 0.05820471094892911 \newline
- 0.01920667012634072 \newline
- 0.12431866468061546 \newline
- 0.0206622901528962 \newline
- 0.09149063683310935 \newline
- 0.03769061799536675 \newline
scale\_random\_interact: 1 \newline
seed: 1234 \newline
stage\_ix\_pop\_dict: \newline
  0: 99995 \newline
  1: 3 \newline
  2: 2 \newline
  3: 0 \newline
  4: 0 \newline
  5: 0 \newline
  6: 0 \newline
  7: 0 \newline
  8: 0 \newline
  9: 0 \newline
  10: 0 \newline
stage\_ix\_to\_stages\_dict: \newline
  0: SUSCEPTIBLE \newline
  1: ASYMPTOMATIC \newline
  2: PRESYMPTOMATIC\_MILD \newline
  3: PRESYMPTOMATIC\_SEVERE \newline
  4: MILD\_SYMPTOMS \newline
  5: SEVERE\_SYMPTOMS \newline
  6: HOSPITALIZED \newline
  7: CRITICAL\_ICU \newline
  8: DEATH \newline
  9: HOSPITALIZED\_RECOVERING \newline
  10: RECOVERED \newline
type: generated \newline
use\_gpu: true \newline
\# for poc testing \newline
poc\_test\_on\_symptoms: false \newline
poc\_test\_start\_date: 0 \newline
poc\_test\_true\_positive: 0.85 \newline
poc\_test\_false\_positive: 0.0 \newline
\# for rtpcr testing \newline
rtpcr\_test\_start\_date: 0 \newline
test\_false\_positive: 0.0 \newline
test\_results\_dates: \newline
- 1 \newline
- 2 \newline
- 3 \newline
test\_results\_dates\_probs: \newline
- 0.3 \newline
- 0.4 \newline
- 0.3 \newline
test\_true\_positive: 0.99 \newline
test\_validity\_days: -1 \newline
\# for DCT \newline
app\_adoption\_rate: 0.4 \newline
use\_app\_age\_dist: false \newline
max\_den\_contact\_days: 7 \newline
poc\_den\_inform\_prob: 1.0 \newline
dct\_poc\_comply\_prob: 0.8 \newline
dct\_rtpcr\_comply\_prob: 0.8 \newline
\# for MCT \newline
poc\_mct\_inform\_prob: 1.0 \newline
max\_mct\_contact\_days: 7 \newline
mct\_recall\_prob: 0.7 \newline
mct\_reachable\_prob: 0.95 \newline
mct\_poc\_comply\_prob: 0.95 \newline
mct\_rtpcr\_comply\_prob: 0.95 \newline
\# for self-quarantine \newline
en\_quarantine\_enter\_prob: 0.8 \newline
mct\_quarantine\_enter\_prob: 0.9 \newline
quarantine\_break\_prob: 0.01 \newline
quarantine\_days: 14 \newline
\# for vaccination \newline
vaccine\_daily\_production: 300 \newline
vaccine\_drop\_prob\_before\_second\_dose: 0.3 \newline
vaccine\_first\_dose\_effectivness: 0.9 \newline
vaccine\_first\_dose\_kick\_in\_days: 14 \newline
vaccine\_first\_dose\_priority: true \newline
vaccine\_second\_dose\_delay: 21 \newline
vaccine\_second\_dose\_effectiveness: 0.95 \newline
vaccine\_shelf\_life: 2 \newline
vaccine\_start\_date: 10 \newline
 \newline
use\_den\_logic: true \newline
use\_gps\_logic: false \newline
use\_mct\_logic: true \newline
use\_hybrid\_logic: false \newline
use\_poc\_test\_on\_ct\_logic: false \newline
use\_rtpcr\_test\_on\_ct\_logic: false \newline
use\_rtpcr\_test\_logic: true \newline
use\_quarantine\_logic: true \newline
use\_vaccination\_logic: false \newline
results\_file\_postfix: CT \newline
 \newline


}

